Q-SHED: Distributed Optimization at the Edge via Hessian Eigenvectors Quantization

Edge networks call for communication efficient (low overhead) and robust distributed optimization (DO) algorithms. These are, in fact, desirable qualities for DO frameworks, such as federated edge learning techniques, in the presence of data and system heterogeneity, and in scenarios where internode communication is the main bottleneck. Although computationally demanding, Newton-type (NT) methods have been recently advocated as enablers of robust convergence rates in challenging DO problems where edge devices have sufficient computational power. Along these lines, in this work we propose Q-SHED, an original NT algorithm for DO featuring a novel bit-allocation scheme based on incremental Hessian eigenvectors quantization. The proposed technique is integrated with the recent SHED algorithm, from which it inherits appealing features like the small number of required Hessian computations, while being bandwidth-versatile at a bit-resolution level. Our empirical evaluation against competing approaches shows that Q-SHED can reduce by up to 60% the number of communication rounds required for convergence.

==> HR_quantization.tex <==
\subsection{Bit allocation with first-order approximation}
In this section, we solve problem (\ref{eq:optPbm}) by applying a first order approximation to the cost function $f(\mathbf{x}_q, q)$. This design choice allows us to solve the optimization problem in closed form. The first order approximation provides intuition in the bit allocation scheme and has the advantage of being computationally cheaper with respect to solving the original problem, which requires multiple executions of an iterative algorithm.

Neglecting the second order terms in the cost function, the optimization problem is then

\begin{equation}\label{eq:optPbmFO}
	\begin{aligned}
		\min_{\mathbf{x}_q, q} \quad & f_1(\mathbf{x}_q, q) = \sum_{i = q+1}^{n}\bar{\lambda}_{q, i}^2 + \sum_{i = 1}^{q}\gamma_{n,q, i}x_i\\
		\textrm{s.t.} \quad & -\sum_{i = 1}^q \log x_i \leq 2(B-q)
	\end{aligned}
\end{equation}

and the optimization problem can be written as in (\ref{eq:optPbm}). Neglecting the set of constraints on the admissible values of $x_i$: $0 < x_i \leq 4$, we can solve the optimization problem in closed form by writing the KKT optimality conditions. Indeed, the following Lemma holds:


	Using the first-order approximation $f_1(\mathbf{x}_q, q)$ of the original cost function, for any $q =1,...n$, the optimal solution of the problem (\ref{eq:optPbmFO}) is
	\begin{equation}
		x_i^* = \frac{\prod_{i = 1}^{q}(\gamma_{n, {q}, i})^{1/q}}{4^{B/q - 1}\gamma_{n, {q}, i}} = \frac{\prod_{i = 1}^{q}(d_q\bar{\lambda}_{q, i} + a(n)\bar{\lambda}_{q, i}^2)^{1/q}}{(d_q\bar{\lambda}_{q, i} + a(n)\bar{\lambda}_{q, i}^2)4^{B/q - 1}}.
	\end{equation}

Indeed, the KKT optimality conditions are:
\begin{equation}
	\begin{aligned}
		\nabla_{\mathbf{x}_q} [f_1(\mathbf{x}_q, q) + \mu (-\sum_{j = 1}^{q} \log_2 x_j - 2(B - q))]_i = 0,
	\end{aligned}
\end{equation}
which is satisfied if and only if 
\begin{equation}
	 \gamma_{n, {q}, i} - \mu\frac{\log_2e}{x_i} = 0
\end{equation}
from which we get
\begin{equation}\label{eq:optMu}
	x_i^* = \frac{\mu}{\gamma_{n, {q}, i}}\log_2e.
\end{equation}
From the explicit expression of the solution, we can get the value of $\mu$ satisfying the constraint on the bit budget with equality:
\begin{equation}
	\begin{aligned}
			\sum_{i = 1}^{q} \log_2 x_i^* = 2(B - q)
	\end{aligned}
\end{equation}
from which we get
\begin{equation}
	\begin{aligned}
		&-q\log\mu - \sum_{i = 1}^{q}\log(\frac{\log_2e}{\gamma_{n, {q}, i}}) = 2(B-q)\\&\iff  \log_2\mu = \frac{1}{q}\sum_{i = 1}^q\log_2(\frac{\gamma_{n, {q}, i}}{\log_2e}) - \frac{2}{q}(B-q)\\&\iff \mu = \frac{\prod_{i = 1}^{q}(\gamma_{n, {q}, i})^{1/q}}{4^{B/q - 1}\log_2e}.
	\end{aligned}
\end{equation}

Hence, the optimal $x_i^*$ can be derived in closed form by plugging the explicit value of $\mu$ in (\ref{eq:optMu})

It easy to see from the above expression that the optimal choice for the quantization intervals is such that $$x_1^* \leq x_2^* \leq \cdots \leq x_q^*$$ which is what we would expect: eigenvectors component corresponding to smaller eigenvectors are quantized with fewer bits with respect to eigenvectors corresponding to higher eigenvalues.

The closed form solution satisfies the positivity constraints, meaning that $x_i^* > 0, \ \forall i = 1, ..., q$, while no guarantee is provided about the bound $x_i <= 4$ that corresponds to $b_i >= 0$. Because of this, some care needs to be taken to apply the first-order approximation closed form solution.






==> VecQuantTechs.tex <==

We suppose to use a spherical vector quantization (SVQ) for the eigenvectors $v_1, ..., v_n, v_i \in \mathbb{R}^n$, meaning that each eigenvector is mapped into $\hat{v}_1, ..., \hat{v}_n$ on the unit sphere. Note that then
\begin{equation}
	\|v_i\| = \|\hat{v}_i\| = 1, \forall i = 1, ..., n.
\end{equation}
We assume that some SVQ is used, with a certain number of bits $N_i$ allocated for each eigenvector $v_i$ and we analyze the quantization distortion analyzing the ‘ideal’ SVQ approach considering ‘spherical cap’ quantization cells, following the approach of \cite{LSVQ}.

The quantized eigenvector $\hat{v}_i$ is therefore a spherical codevector located at the center of a spherical cap. Here, as in~\cite{LSVQ}, we assume that the error vector in quantizing $v_i$ is uniformly distributed in the cell, from which, denoting the chordal distance by 

\begin{equation}
	\|v_i - \hat{v}_i\| = \|\epsilon_i\|
\end{equation}
we can get the distortion as

\begin{equation}\label{eq:distortion}
	\begin{aligned}
		D_{svq, i} = \mathbb{E}[\|\epsilon_i\|^2 | v_i] & = \int_{C_{\hat{v}_i}}p(\epsilon_i)\|\epsilon_i\|^2d\epsilon_i \\& = \frac{\int_0^{\gamma} 2\cdot \sin^2(\frac{\beta}{2})(\sin(\beta))^{n-2}d\beta}{\int_0^{\gamma}(\sin(\beta))^{n-2}d\beta}
	\end{aligned}
\end{equation}
denoting by $C_{\hat{v}_i}$ the surface of the spherical cap. $p(\epsilon_i) = 1/S_{C_{\hat{v}_i}}$ is the uniform probability distribution over the surface $S_{C_{\hat{v}_i}}$ of the cap. For the derivation of (\ref{eq:distortion}), see \cite{LSVQ}.

We now analyze the expected Hessian quantization error by means of the expected squared Frobenious norm:

\begin{equation}
	\begin{aligned}
		e(H, \hat{H}) :&= \mathbb{E}[\|H-\hat{H}\|_{\mathcal{F}}^2|v_1, ..., v_n, \lambda_1, ..., \lambda_n] \\&= \mathbb{E}[tr((H-\hat{H})(H-\hat{H}))|v_1, ..., v_n, \lambda_1, ..., \lambda_n],
	\end{aligned}
\end{equation}
where $tr(\cdot)$ denotes the trace of a matrix.

In the following, we drop the conditioned values to simplify the notation. We get

\begin{equation}\label{eq:esplicitFN}
	\begin{aligned}
		e(H, \hat{H}) &= \mathbb{E}[tr(\sum_{i = 1}^{n}\lambda_i(v_iv_i^\top - \hat{v}_i\hat{v}_i^\top))(\sum_{i = 1}^{n}\lambda_i(v_iv_i^\top - \hat{v}_i\hat{v}_i^\top))]\\& = \mathbb{E}[tr(\sum_{i = 1}^n\lambda_i\delta V_i)(\sum_{i = 1}^n\lambda_i\delta V_i)] = \mathbb{E}[tr(\sum_{i = 1}^n\lambda_i^2\delta V_i\delta V_i) + tr(\sum_{i\neq j}\lambda_i \lambda_j\delta V_i\delta V_j))],
	\end{aligned}
\end{equation}
defining $\delta V_i = (v_iv_i^\top - \hat{v}_i\hat{v}_i^\top)$. We now analyze the first sum in (\ref{eq:esplicitFN}):

\begin{equation}
	\mathbb{E}[tr(\sum_{i = 1}^n\lambda_i^2\delta V_i\delta V_i) ] = \sum_{i = 1}^n\lambda_i^2\mathbb{E}[tr(\delta V_i\delta V_i)].
\end{equation}
The computation requires then to compute the quantity $\mathbb{E}[tr(\delta V_i\delta V_i)]$. Given that $(\delta V_i\delta V_i) = v_iv_i^\top - v_iv_i^\top \hat{v}_i \hat{v}_i^\top -  \hat{v}_i \hat{v}_i^\top v_iv_i^\top + \hat{v}_i\hat{v}_i^\top$, where we have used the fact that $\hat{v}_i^\top\hat{v}_i = 1$.
\begin{equation}
	\mathbb{E}[tr(\delta V_i\delta V_i)] = \mathbb{E}[tr(v_iv_i^\top - v_iv_i^\top \hat{v}_i \hat{v}_i^\top -  \hat{v}_i \hat{v}_i^\top v_iv_i^\top + \hat{v}_i\hat{v}_i^\top)].
\end{equation}

After some calculation, we get
\begin{equation}
	\begin{aligned}
		\mathbb{E}[tr(\delta V_i\delta V_i)] &= 2 + D_{svq, i} - 2(1 + tr(v_iv_i^\top \mathbb{E}[\epsilon_i\epsilon_i^\top])) \\&= D_{svq, i} - 2tr(v_iv_i^\top K),
	\end{aligned}
\end{equation}
where $K = \mathbb{E}[\epsilon_i\epsilon_i^\top])]$. \textbf{The problem} is: what is $tr(v_iv_i^\top K)$ in a spherical vector quantization scheme? Is $K$ diagonal? In that case we have $tr(v_iv_i^\top K) = \sum_{j = 1}^{n}v_{ij}^2k_{jj}$, where $k_{jj} = \mathbb{E}[\epsilon_{ij}^2]$ but what is the value of $k_{jj}$? Note that we only know $D_{svq, i} =  \mathbb{E}[\|\epsilon_i\|^2] = \sum_{j = 1}^{n}\mathbb{E}[\epsilon_{ij}^2]$.

